Certification for Polynomial Systems via Square Subsystems

We consider numerical certification of approximate solutions to a system of polynomial equations with more equations than unknowns by first certifying solutions to a square subsystem. We give several approaches that certifiably select which are solutions to the original overdetermined system. These approaches each use different additional information for this certification, such as liaison, Newton-Okounkov bodies, or intersection theory. They may be used to certify individual solutions, reject nonsolutions, or certify that we have found all solutions.

==> paper_bottom/ag.tex <==
\subsection{Birationally Intersection Index}
\label{subsec:bii}

Associate to each polynomial system $f$ the finite-dimensional vector space $L=\spa_{\CC} \{ f_1, \ldots , f_N \}.$ The \emph{birationally-invariant intersection index}
\[
d_L := \displaystyle\max_{g_1,\ldots , g_n \in L} \# \variety (g_1,\ldots , g_n)
\]
counts the number of excess solutions for a generic squaring up of $f.$ This number can be computed in terms of certain intrinsic quantities associated to $L$---chiefly, the \emph{volume of a Newton-Okounkov body} associated to this subspace.

General facts concerning intersection indices and Newton-Okounkov bodies~\cite{KK12,KK10}.
Though it is substantially more general than we need, we first recall the following simplified definition of the intersection index for subspaces of rational functions on an irreducible variety $X.$ 

\begin{defn}(\cite[Definition 4.5]{KK12})
Let $X$ be an $n$-dimensional irreducible variety with singular locus $X_{sing}.$ For $(L_1, L_2, \ldots , L_n)$ an $n$-tuple of finite-dimensional complex subspaces of the function field $\CC (X),$ let $\bs{L} = L_1 \times L_2 \times \cdots \times L_n$ and define
\[
U_{\textbf{L}} = \{ x\in X \setminus X_{sing} \mid \displaystyle\cup_{i=1}^n L_i \subset \ocal_{X,x}  \},
\]
\[
Z_{\textbf{L}} = \displaystyle\bigcup_{i=1}^n \{ x\in U_{\bs{L}} \mid f(x) =0 \, \, \forall  f\in L_i\, \,  \}.
\]
The solutions to the system $g_1(x)=g_2(x)=\cdots g_n(x)$ on $U_{\textbf{L}} \setminus Z_{\textbf{L}}$ are all non-singular for generic $g=(g_1,\cdots , g_n)\in \bs{L},$ and their number is independent of the choice of $g.$ The common number defines the intersection index $[L_1,L_2,\ldots , L_n].$ 
\end{defn}
For proofs that the intersection index is well-defined (in somewhat fuller generality), see~\cite[Sections 4 \& 5]{KK10}.

In all cases of interest for this work, we take $X=\CC^n$ and consider the \emph{unmixed} case in which $\bs{L}=L\times L \times \cdots \times L$---moreover, we assume throughout that $L\subset \CC [x_1,\ldots , x_n].$ We hence denote the intersection index by $d_L,$ and note that $U_{\bs{L}} = \CC^n,$ while $Z_{\bs{L}}$ is simply the variety defined by $L.$

\begin{figure}
\label{fig:od_circles}
\begin{center}
\includegraphics[width=6cm]{od_circles.eps}
\end{center}
\caption{Intersections of $3$ circles}
\end{figure}
\begin{example}
\label{ex:circ_intro}
The equation of a complex circle in $\CC^2$ has the form
\[
a (x^2+y^2) + b x + cy +d =0,
\]
with coefficients $a,b,c,d \in \CC.$ Two distinct circles will intersect in at most two isolated points in $\CC^2,$  with equality when their coefficients are generic.

For concreteness, consider the circles defined by
\[
f(x,y)=x^2+y^2-4 \, \, \,  \, \, g(x,y) = x^2 + y^2 -2x - 2y.
\]
The zero-locus of $f(x,y)=g(x,y)=0$ in $\CC^2$ consists of two points. Intersecting this locus with a third circle may result in either $2,1$ or $0$ points. The possibilities are realized by intersecting with $h_i(x,y)=0,$ where \blue{$h_2(x,y)=x^2+y^2-4x-4y+4$}, \orange{$h_1(x,y)=x^2+y^2-6x+2y+8$}, and \red{$h_0(x,y)=x^2+y^2-6x+7$}, respectively, as depicted in Figure~\ref{fig:od_circles}.

Squaring up the systems $f(x)=g(x)=h_i(x)=0$ with generic coefficients yields a system defined by two circles. Thus, letting $L_i=\spa_{\CC } \{ f,g,h_i \}$ for each $i=0,1,2,$ the intersection index associated to each squared-up system is given by $[L_i,L_i]=2-i.$

\end{example}

Computation of $d_L$ is generally difficult, but is somewhat facilitated facilitated by considering the associated graded $\CC$-algebra
\[
A_L := \displaystyle\bigoplus_{k=0}^{\infty} t^k L^k \subset \CC (X)[t].
\]
Associate to this algebra, and a fixed valuation $v: \CC (X) \to \ZZ^n ,$ the semigroup
\[
S(A_L,v):=v_t(A_L \setminus \{ 0 \} ),
\]
where $v_t:\CC (X)[t] \to \ZZ^n \times \ZZ$ is the extended valuation defined by
\[
v_t(a_n t^n + \cdots + a_1 t + a_0 )=\left(v(a_n),n\right).
\]
\begin{comment}
Associated to the semigroup $S(A_L,v)$ are the following objects:
\begin{itemize}
\item[i)] CONE
\item[ii)] group
\item[iii)] projection
\item[iv)] nobody.
\end{itemize}

\begin{example}[Sweedler+Robbiano 2]
\label{ex;sw_11}
Consider $L=\spa_\CC \{ x, xy-y^2 , xy^2 \}.$ For any valuation induced by a term order, the given polynomials form a triangular basis. 
\end{example}
\end{comment}


==> paper_bottom/alpha.tex <==
\label{sec:appx-square}

We begin with our operational definition of an approximate solution.

\begin{defn}
\label{defn::appx-solution}
A $\delta$-\emph{approximate solution} for a polynomial system $f\in (\CC [x_1,\ldots , x_n])^N$ is a triple $(\hat{\zeta}, \delta , \mathcal{N}_f),$ where $\hat{\zeta }\in \mathbb{C}^n,$ $\delta \in \RR_{>0},$ and $\mathcal{N}_{f} : U \to \CC^n$ is a map defined on some $U \subset \CC^n$ such that:
\begin{itemize}
\item[1)] There exists $\zeta \in \variety (f)$ such that $|\zeta - \hat{\zeta} | < \delta $
\item[2)] All iterates $\mathcal{N}_f^k (\hat{\zeta} )$ are defined and the following refinement property holds: for any $\epsilon >0,$ we have $\norm{\mathcal{N}_f^{k} (\hat{\zeta }) - \hat{\zeta }} < \epsilon $ for all $k$ sufficiently large.
\end{itemize}
\end{defn}
Here $\norm{\cdot}$ indicates the usual Hermitian norm on $\CC^n$---any metric on $\CC^n$ will yield a comparable definition. We abusively refer to $\hat{\zeta}$ as an approximate solution when the procedure $A$ is understood.

\begin{remark}
  \label{remark::field}
  For all examples considered in this paper, the system $f$ and the solution $\hat{\zeta }$ are defined over the rationals $\mathbb{Q}$ or the Gaussian rationals $\QQ [i].$ Since numerical solvers typically output floating point results, care must be taken to control rounding errors when computing certificates. One option for certification procedures is to perform all subsequent operations in rational arithmetic. Interval and ball arithmetic give yet another approach (cf.~Example \ref{ex:interval}.) A ``certificate'' obtained without controlling rounding errors may still be of practical value; following~\cite{HS12}, we call this a \emph{soft certificate.} 

  \end{remark}
  
  \begin{remark}
  \label{remark::computability}
In all examples considered, the map $\mathcal{N}_f$ in Definition~\ref{defn::appx-solution} restricts to a computable function $\mathcal{N}_{f,\QQ} : U \cap \QQ[i]^n \to \QQ[i]^n$ We take a naive approach to questions of computability, but we do not rely on special features of non-standard models of computation such as the Blum-Shub-Smale machine (cf.~\cite{BCSS}.)
\end{remark}

An easy consequence of Definition~\ref{defn::appx-solution} is that $\mathcal{N}^k (\hat{\zeta } ) \to \zeta $ as $k\to \infty .$ In practice, we wish to quantify the rate of convergence. This motivates the next definition.
\begin{defn}
\label{defn::effective-appx-solution}
An \emph{effective approximate solution} consists of an approximate solution $(\hat{\zeta},\delta, A)$ together with a rate-determining function $r: \mathbb{R}_{>0} \to \mathbb{N}$ such that for each $\epsilon >0$ we have $\norm{\mathcal{N}_f^{k} (\hat{\zeta }) - \hat{\zeta }} < \epsilon $ for all $k\ge r(\epsilon ).$ We say the rate of convergence is of order $\epsilon (k)$ if $\norm{\mathcal{N}_f^{j} (\hat{\zeta }) - \hat{\zeta }} < \epsilon (k)$ for all $j\ge r(\epsilon (k)).$ 
\end{defn}

For the special case of $\epsilon (k) = 2^{- 2^{O(k)} },$ we say that convergence is \emph{quadratic.} This implies that each application of $N_g(\cdot)$ roughly doubles the number of significant digits.

In the case of a \emph{square} system $g\in (\CC [x_1, \ldots , x_n])^n,$ existing certification techniques are based on Newton's method and typically exhibit quadratic convergence. We review the main results in the context of Definitions~\ref{defn::appx-solution} and~\ref{defn::effective-appx-solution}.

\begin{example}
  % alpha
  \label{ex::alpha}
Smale's $\alpha$-theory gives a criterion for approximate zeros based on Newton's method. For $k\in\NN$, let $S^k\CC^n$ be the $k$th symmetric power of $\CC^n$.
This has a norm $\norm{\cdot }$ dual to the standard unitarily invariant norm on homogeneous polynomials, and which
satisfies $\|z^k\|\leq \|z\|^k$, for $z\in\CC^n$. 
The $k$-th derivative of $g$ at $\zeta$ is a linear map $\diff{g}{k}{\zeta}: S^k(\CC^n) \to \CC^n$ with operator norm,
%
 \begin{equation}
  \label{op_norm}
   \norm{ \diff{g}{k}{\zeta} }\ :=\  \displaystyle\max_{
    \substack{
      w \in S^k\CC^n
      \\[0.25em]
      \norm{w}=1}
      }
    \norm{\diff{g}{k}{\zeta} \, (w)}\,.
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{defn}
\label{alpha_beta_gamma}
With $g$ as above and $\hat{\zeta}\in \CC^n$ a point where $Dg(\hat{\zeta})$ is invertible,
\begin{align*} 
  \alpha (g,\hat{\zeta})\ &:=\ \beta(g,\hat{\zeta}) \cdot \gamma (g,\hat{\zeta})\  \text{, \ where}\\
  \beta (g,\hat{\zeta})\ &:=\ \norm{\hat{\zeta} - N_g (\hat{\zeta})}
                           \ =\  \norm{ Dg(\hat{\zeta})^{-1} g(\hat{\zeta})}\  \text{  and}\\
  \gamma (g,\hat{\zeta})\ &:=\
                 \sup_{k\geq 2}\left\|\frac{Dg(\hat{\zeta})^{-1}\diff{g}{k}{\hat{\zeta}} }{k!}\right\|^{\frac{1}{k-1}}  .
\end{align*}
Notice that $\beta(g,\hat{\zeta})$ is the length of a Newton step at $\hat{\zeta}$.
\end{defn}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{prop} [{\cite[p.~160]{BCSS}}]
  \label{prop:alpha}
  Let $g$ be a square polynomial system and $\hat{\zeta}\in\CC^n$.
  If
  \[
    \alpha(g,\hat{\zeta})\ <\ \frac{13-3\sqrt{17}}{4}\ \approx\ 0.15767078\,,
  \]
  then $\hat{\zeta}$ is $2 \beta( g, \hat{\zeta} )$-approximate solution to $g$.
\end{prop}

  
\end{example}

\begin{example}
% Kantorovich
\red{TODO: say something about Kantorovich's analysis of Newton's method}
\end{example}

\begin{example}
\label{ex:interval}
Approximate solutions may also be understood within the general program of interval and ball arithmetics. Both paradigms rely on defining arithmetic operations on intervals or balls and have the feature of being definable in either exact or floating point of arithmetic. In general, operations are on intervals represent \emph{enclosures}: thus, in exact interval arithmetic, we define the sum by $[a,b]+[c,d]=[a+c,c+d].$ For floating point arithmetic, we may either accept a soft certificate or control rounding errors rigorously when defining arithmetic operations. We refer to the sources \red{list some sources}. One an interval or ball arithmetic is defined, an interval or ball version of Newton's method can be studied. \red{cite relevant sources. Explain that we get appx zero according to our definition by taking midpoints} 
\end{example}

Our approach to over-determined certification rests on the ability to perform two tasks with approximate solutions to a square system $g:$

\begin{itemize}
\item[1)] \emph{separation}---if $\hat{\zeta }$ and $\hat{\zeta }'$ are approximation solutions to $g,$ how can we decide if the associated solutions are the same?
\item[2)] 
\end{itemize}

Theorem 6 and Remark 9 of~\cite[Ch.~8]{BCSS} give a refined version of Proposition~\ref{prop:alpha} that provides a
certificate that two approximate solutions have the same associated solution.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{prop}
  \label{prop:same}
  Let $g$ be a square polynomial system and $\hat{\zeta}\in\CC^n$ an approximate solution to $g$ with associated solution
  $\zeta$ and suppose that $\alpha(g,\hat{\zeta})<0.03$.
  If $\hat{\zeta}'\in \CC^n$ satisfies
  \[
    \| \hat{\zeta} - \hat{\zeta}'\|\ <\ \frac{1}{20\gamma(g,\hat{\zeta})}\,,
  \]  
  then $\hat{\zeta}'$ is a $2\beta (g, \hat{\zeta })$-approximate solution to $g$ with associated solution $\zeta$.
\end{prop}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Propositions~\ref{prop:alpha} and~\ref{prop:same} enable algorithms to certify that a set of approximate solutions have
pairwise disjoint associated solutions.
For example, Proposition~\ref{prop:alpha} implies a separation bound.
If $\hat{\zeta}_1$ and $\hat{\zeta}_2$ are approximate solutions to $g$ with
%
 \begin{equation}\label{eq:separation}
  \| \hat{\zeta}_1 - \hat{\zeta}_2\|\ \geq\ 2(\beta(g,\hat{\zeta}_1)+\beta(g,\hat{\zeta}_2))\,,
 \end{equation}
%
then their associated solutions are distinct.
Given an approximate solution $\hat{\zeta}$ with associated solution $\zeta$ such that $Dg(\zeta)$ is invertible, the
sequence $\beta(g, N^k_g(\hat{\zeta}))$ converges to zero.
As derivatives are continuous, $\gamma(g, N^k_g(\hat{\zeta}))$ is bounded, so that $\alpha(g, N^k_g(\hat{\zeta}))$ converges
to zero.
Thus we may refine approximate solutions $\hat{\zeta}_1$ and $\hat{\zeta}_2$ to $g$ with Newton iterations 
until either~\eqref{eq:separation} holds---so they represent distinct solutions to $g$---or
Proposition~\ref{prop:same} applies and they represent the same solution.
Having obtained representatives of distinct solutions to $g$, we may refine them to obtain a pairwise disjoint collection
of balls containing each, as well as their associated solutions to $g$.
We summarize this discussion.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{prop}
  \label{prop:separating}
 Given a square system $g$ with approximate solutions $S'$, we may compute a set $S$ of refined approximate solutions and a
 set $B$ of pairwise disjoint balls centered at elements of $S$ such that each ball contains the solution to $g$ associated
 to its center.
\end{prop}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Suppose now that $f$ is an overdetermined polynomial system, and that $\hat{\zeta},\zeta\in\CC^n$ with
$f(\zeta)=0$. 
We say that $\hat{\zeta}$ is an \emph{approximate solution} to $f$ with \emph{associated solution} $\zeta$ if there is a
square subsystem $g$ of $f$ such that  $\hat{\zeta}$ is an approximate solution to $g$ with
associated  solution $\zeta$. As we generally only know $f,g,$ and $\hat{\zeta },$ establishing that the associated zero $\zeta $ is a solution to $f$ seems difficult \emph{a priori}. On the other hand, $\alpha$-theory provides a simple certificate that $\zeta $ is \emph{not} a solution to $f.$

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{prop}
  \label{prop:reject}
  Suppose that $g$ is a square subsystem of $f=(f_1,\dotsc , f_N)$ and that $\hat{\zeta }$ is an approximate solution to
  $g$ with associated solution $\zeta$.
  Consider
  \begin{equation}
    \label{eq:taylor_bound}
    \delta (f, g, \hat{\zeta })\ :=\  \displaystyle\max_{1\le j \le N}
      \Big( \,
        |f_j (\hat{\zeta })| - \displaystyle\sum_{k=1}^{\deg f_j}
        \displaystyle\frac{\norm{\diff{f_j}{k}{\hat{\zeta }}}}{k!}
        \cdot \big( 2 \, \beta (g,\hat{\zeta }) \big)^k
      \Big)\ .
  \end{equation}
  If $\delta (f,g, \hat{\zeta} ) >0$ and $\|\hat{\zeta}-z\|<2 \beta (g,\hat{\zeta })$, then $f(z)\neq 0$.
  In particular, $f(\zeta )\ne 0$.
\end{prop}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
 This follows from Proposition~\ref{prop:alpha} and Taylor expansion.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In practice, we estimate the operator norms of the higher derivatives, as explained in~\cite[\S I-3]{SS93}
and~\cite[\S1.1]{HS12}. 


==> paper_bottom/bases.tex <==
\subsection{Khovanskii bases and triangular bases}
\label{subsec:bases}
\red{Original reference for KB is Kaveh and Manon?} 
\begin{defn}
Given a valuation $v$ on $\CC (X),$ a \emph{Khovanskii basis} for $A_L$ is a finite set $\bcal \subset A_L$ such that $v_t(\bcal )$ generates the semigroup $S(A_L,v).$ 
\end{defn}
Of particular interest is the case in which the subspace $L$ itself contains a Khovanskii basis. It turns out that this is relatively easy to check.
\begin{defn}
Let $L$ be a subspace of $\CC (X).$ A \emph{triangular basis} for $L$ with respect to the valuation $v:\CC (X)\to \ZZ^n$ is a subset $\bcal \subset L$ such that $v(f_i) \ne v(f_j)$ for any two distinct $f_i,f_j\in \bcal .$ 
\end{defn}
In our setting, where $X=\CC^n,$ computing a triangular basis for the subspace $L=\spa_{\CC } \{ f_1, \ldots , f_N \} \subset \CC [x_1,\ldots , x_n]$ reduces to computing a row-echelon form for a $N \times |\supp (L) |$ matrix, where $\supp (L)$ is the set of monomials supported on $L.$ 
\begin{prop}
\label{prop:khovanskii_L}
  For fixed valuation $v,$ a triangular basis for $L$ forms a Khovanskii basis for $A_L$ if and only if $2v(L)=v(L^2).$
\end{prop}
\begin{proof}
$\Rightarrow $ Note first that for arbitrary $L_1, L_2$, we have
  \begin{equation}
    \label{eq:val_inclusion}
    v(L_1 ) + v(L_2) \subset v(L_1 L_2)
  \end{equation}
  In particular, $2v(L) \subset v(L^2).$ If this inclusion is strict, then $v_t (\CC + t L)$ generates a semigroup strictly contained in $S(A_L,v).$\\$\Leftarrow $ More generally, suppose that
  \[
v(L^d)=d \, v(L)
\]
for some $d\in \NN.$ Then
\begin{align*}
  v(L^{d+1}) &\subset v(L^d) + v(L) \tag{\eqref{eq:val_inclusion}}\\
  &= (d+1) \, v(L),
\end{align*}
and a similar induction gives that $v(L^{d+k})=(d+k) \, v(L)$ for all $k\ge 0.$ Hence
\[
v(L) \cup v(L^2) \cup \cdots \cup v(L^d)
\]
forms a Khovanskii basis. Specializing to $d=1$ gives the result. 
\end{proof}
Proposition 


\begin{example}[Sweedler+Robbiano 2]
\label{ex;sw_11}
\red{Problematic example}
Consider $L=\spa_\CC \{ x, xy-y^2 , xy^2 \}.$ For any valuation induced by a term order with $y<x,$ the given polynomials form a triangular basis. 
\end{example}


\red{TODO: Resolve problematic example, address case where $2 \, v(L) \subsetneq v(L^2).$ }


==> paper_bottom/certInd.tex <==
%Certifying Individual Solutions


The consequences of $\alpha$-theory and Proposition~\ref{prop:reject} furnish a certification procedure for overdetermined
systems in the following setting---Suppose we are given a system $f$, a square subsystem $g$ where we know, by some means,
%
%  Frank:  For simplicity, I removed the \leq.  That can be handled in the full paper ?
%
If we can certify $d$ solutions to $g$ which are not solutions to $f,$ then any other
solutions to $g$ must be solutions to $f.$

\begin{algorithm}[Certifying individual solutions]\label{alg:ind}$ $\\
  \textbf{Input:} $(f,g, d, S )$
  \begin{itemize}%[topsep=0pt,parsep=0pt]
  \item[] $f$ --- a polynomial system
  \item[] $g$ --- a square subsystem of $f$
  \item[] $d \in \NN$ satisfying \eqref{eq:bound}
  \item[] $S = \{ \hat{\zeta_1 }, \ldots , \hat{\zeta_m} \}$ --- pairwise distinct approximate solutions to $g$ 
  \end{itemize}
  \textbf{Output:} $T\subset S,$ a set of approximate solutions to $f$
  \begin{algorithmic}
    \STATE Initialize $R\gets \emptyset $
    \STATE{\textbf{for } $j=1,\dotsc, m$ \textbf{ if } $\delta (f,g,\hat{\zeta_j}) >0$ \textbf{ then }
              $R\gets R \cup \{ \zeta_j \}$ }
    \STATE{\textbf{if } $(\# R == d)$ \textbf{ then } $T\gets S\smallsetminus R$ \textbf{, else } $T\gets \emptyset $}
      \RETURN $T$
  \end{algorithmic}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{remark}
\label{remark:boundd}
\emph{A priori,} we only need to know that $d \ge \# \left( \variety (g) \setminus \variety (f)\right)$---if the inequality is strict, we necessarily return an empty set.
\end{remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{thm}
  \label{thm:ind}
  Suppose that $f,g,d,S$ are valid input for Algorithm~\ref{alg:ind}.
  Then its output consists of approximate solutions to $f$.
\end{thm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
  If $T$ is empty there is nothing to prove.
  Otherwise, there are $d$ distinct solutions to $g$ associated to points of $R$---by Proposition~\ref{prop:reject}, these
  are not solutions to $f$. 
  Since the solutions associated to points of $T$ are disjoint from those associated to points of $R$, by assumption
  and~\eqref{eq:bound} they associate to solutions to $f$. 
  % F: I think that it is best to have punctuation in text mode.
\end{proof}
%

Perhaps the main difficulty in applying Algorithm~\ref{alg:ind} is obtaining the correct number $d$ beforehand.
When we square up by random matrix as in~\eqref{eq:mat}, this number is given by a birationally-invariant intersection
index over $\CC^n$.
We summarize the basic tenets of this theory as developed in~\cite{KK10,KK12}.
%Though it is substantially more general than we need, we first recall the following simplified definition of the
%intersection index for subspaces of rational functions on an irreducible variety $X$ of dimension $n$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\begin{defn}(\cite[Def.~4.5]{KK12})
  Let $X$ be an $n$-dimensional irreducible variety over $\CC$ with singular locus $X_{sing}$.
  For an $n$-tuple  $(L_1, L_2, \dotsc , L_n)$ of finite-dimensional complex subspaces of the function field $\CC (X)$, let
  $\bs{L} = L_1 \times L_2 \times \cdots \times L_n$, and define 
\[
   U_{\textbf{L}}\ :=\ \{ z\in X \setminus X_{sing} \mid  L_i \subset \calO_{X,z} \mbox{ for }i=1,\dotsc,n \}\,,
\]
the set of smooth points where every function in each subspace $L_i$ is regular, and  
\[
   Z_{\textbf{L}}\ :=\  \bigcup_{i=1}^n \{ z\in U_{\bs{L}} \mid f(z) =0 \ \ \forall  f\in L_i\, \}\,,
\]
the set of basepoints of $\bs{L}$. 
For generic $g=(g_1,\dotsc , g_n)\in \bs{L}$, all solutions to the system $g_1(z)=\cdots = g_n(z)=0$ on
$U_{\textbf{L}} \smallsetminus Z_{\textbf{L}}$ are nonsingular and their number is independent of the choice of $g$.
The common number is the birationally invariant intersection index $[L_1,L_2,\ldots , L_n]$. 
\end{defn}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

These claims are proven in~\cite[Sections 4 \& 5]{KK10}.
For our purposes, $X=\CC^n$ and $\bs{L}=L\times \cdots \times L$ where $L\subset \CC [z_1,\ldots , z_n]$
is the linear space spanned by the polynomials in our system $f$.
Write $d_L$ for this self-intersection index, note that $U_{\bs{L}} = \CC^n$, while $Z_{\bs{L}}=\variety (f)$.
Thus~\eqref{eq:bound} holds for general square subsystems of $f$, taking $d=d_L$.\medskip 

Let  $\nu \colon \CC (X)^\times \to (\ZZ^n , \prec )$ be a surjective valuation where $\prec $ is some fixed total order on
$\ZZ^n$.
For example, $\nu$ could restrict to the exponent of the leading monomial in a term order $\prec$ on $\CC[x_1,\dotsc,x_n]$.
We attach to $(L,\nu )$ the following data:
\begin{itemize}
\setlength\itemsep{0.3em}
% \item $A_L = \oplus_{k=0}^{\infty } t^k L^k,$ a graded subalgebra of $k(X)[t].$
% \item 
\item $A_L=\displaystyle\bigoplus_{k=0}^\infty t^k L^k$---a graded subalgebra of $\CC (X)[t].$ 
\item $S(A_L,\nu ) = \{ (\nu (f), k) \mid f \in L^k \text{ for some } k \in \NN \}$, a sub-monoid of $\ZZ^n \oplus \NN$
  associated to the pair $(L,\nu ),$ where $L^k$ is the $\CC$-span of $k$-fold products from $L$.
  This is the \demph{initial algebra} of $A_L$ with respect to the extended valuation $\nu_t \colon\CC (X)(t)^\times \to
  (\ZZ^n \oplus \ZZ ,\prec_t)$ defined by $\nu_t (f_k\,t^k +\cdots  + f_0 ) \mapsto \left(\nu (f_k) , k \right),$ where
  $\prec_t$ is the \emph{levelwise order} defined by 
\[
    (\alpha_1 , k_1)\ \prec_t\ (\alpha_2, k_2) \quad \text{ if }
    \quad  k_1\ >\ k_2 \quad \text{ or }
    \quad k_2\ =\ k_1 \  \text{and} \quad \alpha_1\ \prec\ \alpha_2\,.
\]
\item $\ind (A_L , \nu )$---the index of $\ZZ \, S(A_L,\nu ) \cap \left( \ZZ^n \times \{ 0\} \right)$ as a subgroup of $\ZZ^n \times \{ 0 \}$.
\item $\overline{\Cone (A_L,\nu )}$---the Euclidean closure of all $\RR_{\ge 0}$-linear combinations from $S(A_L, \nu ).$
\item $\Delta (A_L,\nu )= \overline{\Cone (A_L,\nu )}\cap (\RR^{n}\times\{1\})$---the \demph{Newton-Okounkov body.}
\end{itemize}\smallskip

The linear space $L$ induces a rational \demph{Kodaira map}
\[
  \Psi_L\ \colon\ X\ --\to\ \PP (L^*)\qquad
  z\ \mapsto\ \big[ f \mapsto f(z) \big]\,,
\]
with the section ring $A_L$ the projective coordinate ring of the image.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{prop}[{{\cite[Thm.~4.9]{KK12}}}]
\label{prop:kk}
  Let $L$ be a finite-dimensional subspace of $\CC (X)$.
  Then
\[
  d_L\ =\ \displaystyle\frac{n! \, \deg \Psi_L}{\ind (A_L,\nu )} \cdot \Vol \, \Delta (A_L, \nu).
\]
Here, $\Vol$ denotes the $n$-dimensional Euclidean volume in the slice $\RR^n \times \{1 \}$.
\end{prop}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In our setting, where $X=\CC^n$ and $L= \spa_\CC \{ f_1,\ldots , f_N \},$ the Kodaira map $\Psi_L $ is 
$z \mapsto [f_1(z) : f_2(z) : \cdots : f_N (z)]$.
Thus, if need be, $\deg \Psi_L$ may be computed symbolically.
The main difficulty in applying Proposition~\ref{prop:kk} is that it may be hard to determine the 
Newton-Okounkov body, as the monoid $S(A_L,\nu )$ need not be finitely generated.
This leads us to the notion of a finite Khovanskii basis~\cite{KM16}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{defn}
  \label{def:khovanskii}
  A \emph{Khovanskii basis} for $(L,\nu)$ is a set $\{a_i\mid i\in I\}$ of generators for the algebra $A_L$ whose values
  $\{\nu_t (a_i)\mid i\in I\}$ generate the monoid $S(A_L, \nu )$.
  If $<$ is a global monomial order on $k[z_1,\ldots , z_n],$ taking lead monomials defines a valuation
  $\nu\colon k[z_1,\ldots , z_n] \to (\ZZ^n,\prec)$, where $\prec $ is the reverse of $<$.
  A Khovanskii basis with respect this valuation is commonly known as a \emph{SAGBI basis}~\cite{KM89,RS90}. 
\end{defn}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

When the monoid  $S(A_L,\nu )$ is finitely generated, there is a finite Khovanskii basis for $(L,\nu)$. When this occurs, we may compute the Khovanskii basis via a binomial-lifting/subduction algorithm such as described
in~\cite{RS90} or~\cite[Ch.~11]{Stu96}.

\begin{example}
We consider an ``illustrative example'' of an overdetermined system from~\cite{AHS18}: $$
\left(
\begin{array}{c}
f_1(z_1,z_2,z_3)\\
f_2(z_1,z_2,z_3)\\
f_3(z_1,z_2,z_3)\\
f_4(z_1,z_2,z_3)
\end{array}
\right)
= \left(
\begin{array}{c}
\demph{{z}_{1}^{2}}+{z}_{2}^{2}-1,\,\\
\demph{-{16}\,{z}_{2}^{2}}+{8}\,{z}_{1}+{17
      },\,\\
      \demph{-{z}_{2}^{2}+{z}_{1}}-{z}_{3}-1,\,\\
      \demph{64\,{z}_{1}{z}_{2}}+{16}\,{z}_{2}
      \end{array}
            \right)
      $$
The square subsystem defiened by $f_1=f_2=f_3=0$ has two singular solutions, and $f_4$ is the Jacobian determinant of this subsystem. Let $<$ be the graded reverse lexicographic ordering with $z_1>z_2>z_3$ and $L= \spa_\CC \{ f_1, f_2, f_3, f_4 \}.$ We observe that the initial terms of $tf_1, \ldots, tf_4 \in A_L$ under the induced order $<_t$ are given by $t\,{z}_{1}^{2},\,{-{16}\,t\,{z}_{2}^{2}},\,{-t\,{z}_{2}^{2}},$ and $64 t\,{z}_{1}{z}_{2}.$ The lattice points corresponding to these monomials comprise the first level $S(A_L, \nu ) \cap (x_4 =1)$ and lie in the linear subspace of $\RR^3 \times \{1 \} $ defined by  $x_3=0.$ We see that the inner approximation to the Newton-Okounkov body $\Delta (A_L, \nu )$ given by the first level has $3$-dimensional volume $0.$ However, there exists $x\in S( A_L, \nu )$ with $x_3\ne 0$:
      \begin{eqnarray*}
512\,t^{2}\demph{{z}_{1}^{2}{z}_{3}}+6656\,t^{2}{z}_{1}{z}_{3}-6400\,t^{2}{z}_{3
      }^{2}+14000\,t^{2}{z}_{1}-26368\,t^{2}{z}_{3}-27125\,t^{2} \\
      = t^2 \, (64\,{f}_{1}{f}_{2}-21\,{f}_{2}^{2}-512\,{f}_{1}{f}_{3}+768\,{f}_{2}{f}_{
      3}-6400\,{f}_{3}^{2}+\tfrac{1}{8}\,{f}_{4}^{2}) \in A_L,
\end{eqnarray*}
giving
$$x:=\left(\begin{array}{c} 2\\ 0\\ 1 \\ 2 \end{array} \right) \in S(A_L).$$ This element of $A_L$ was obtained by the previously mentioned binomial-lifting/subduction algorithm---carrying this out further, we can verify that this new element together with the original generators give a finite Khovanskii basis for $A_L.$ It follows that
$$\Delta (A_L, <_t) = \conv
\Bigg(
\left( \begin{array}{c} 1 \\ 0 \\ 0 \\1\end{array} \right),
\left( \begin{array}{c} 0 \\ 2 \\ 0 \\1\end{array} \right),
\left( \begin{array}{c} 1 \\ 1 \\ 0 \\1\end{array} \right),
\left( \begin{array}{c} 2 \\ 0 \\ 0 \\1\end{array} \right),
\left( \begin{array}{c} 1 \\ 0 \\ 1/2 \\1\end{array} \right)
\Bigg)
$$
and $\Vol (A_L) = 1.$ We also have that $\deg \Psi_L = 2$ and $\ind (A_L)=1.$ Thus, we have $[L,L,L]=2,$ giving a total root count of $4$ after squaring up $f.$
\end{example}


==> paper_bottom/certSet.tex <==
% Certifying a set of solutions

We give a second algorithm using $\alpha$-theory to certify solutions to an overdetermined system $f$ to solve Problem 2.
Suppose that we have an overdetermined system $f$ that is known to have $e$ solutions whose square subsystems are
known to have $d$ solutions.
While we could apply Algorithm~\ref{alg:ind} to certify approximate solutions to $f$, we
propose an alternative method to solve this problem.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[Certifying a set of solutions]\label{alg:set}$ $\\
  \textbf{Input:} $(d,e,f,g,S,B)$
  \begin{itemize}%[topsep=0pt,parsep=0pt]
  \item[] $e\leq d$ --- integers
  \item[] $f$ --- a polynomial system with $e$ solutions
  \item[] $g, g'$ --- two square subsystems of $f$
  \item[] $S= \{ \hat{\zeta_1}, \ldots , \hat{\zeta_d} \}$ --- a set of $d$ distinct approximate solutions to $g$
  \item[] $B= \{ B(\hat{\zeta_1}, \rho_1 ) , \,  \ldots ,\, B(\hat{\zeta_d}, \rho_d) \} $
    --- a set of separating balls as in Proposition~\ref{prop:separating} 
  \item[] $S'$ --- a set of $d$ distinct approximate solutions to $g'$
  \end{itemize}
  \textbf{Output:} $T\subset S$, a set of approximate solutions to $f$
  \begin{algorithmic}[1]
    \STATE Initialize $T \gets \emptyset $
\STATE   $r\gets \displaystyle\min_{1\le i < j \le d } \, \Big( \| \hat{\zeta}_i- \hat{\zeta}_j\| - (\rho_i + \rho_i) \, \Big)$
\FOR{ \indent $\hat{\zeta}'\in S'$ }
\STATE{\textbf{repeat } $\hat{\zeta }' \gets N_{g'} (\hat{\zeta} ')$ \textbf{ until } $2\, \beta (g', \hat{\zeta} ')< r/3$}
\STATE{ $\rho ' \gets 2 \, \beta (g', \hat{\zeta} ')$}
\STATE{\textbf{for } $j=1, \, \ldots , d$ \textbf{ if } $B(\hat{\zeta_j}, \rho_j)\cap B '(\hat{\zeta }', \rho ') \ne \emptyset $ \textbf{ then } $T\gets T \cup \{ \hat{\zeta_j } \}$}
\ENDFOR
    \STATE{\textbf{if } $\big(\#T == e \, \big)$, then \textbf{return } $T$ \textbf{, else }\textbf{ return } FAIL}
  \end{algorithmic}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Note that the intersection of balls in line 6 is non-empty if and only if
\[
    \rho ' + \rho_j\ >\ \norm{\hat{\zeta_j}- \hat{\zeta}'}\ ,
\]
so this condition may be decided in rational arithmetic if a hard certificate is
desired.

\begin{thm}
  \label{thm:set}
  Let $f$ be a system of polynomials having $e$ solutions whose general square subsystems have $d$ solutions.
  Then Algorithm~\ref{alg:set} either returns FAIL or it returns a set $T$ of approximate solutions to $f$ whose associated
  solutions are all the solutions to $f$.
\end{thm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As with Algorithm~\ref{alg:ind}, while the hypotheses appear restrictive, they are natural from an intersection-theoretic
perspective, and are satisfied by a large class of systems of equations. We explain one such family coming from Schubert calculus in Section~\ref{subsec:schubertExample}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\begin{proof}
  Since the balls $B(\hat{\zeta}_i,\rho_i)$ are pairwise disjoint, the quantity $r$ is positive.
  Thus the refinement of each approximate solution $\hat{\zeta}'$ on line 4 terminates.
  Having refined each $\hat{\zeta } ' \in S',$ note that $B(\hat{\zeta } ' , \rho ')$ can intersect at most one ball from
  $B$. 
  Now, if $\zeta_1, \ldots , \zeta_e$ are the solutions to $f$, then we must have that some $\hat{\zeta_{i_j}}$ is
  associated to each $\zeta_j$ for some indices $1 \le i_1 < i_2 < \cdots < i_e \le d$.
  Thus, if $T$ has $e$ elements, then the only solutions to $g$ associated to $T$ are also solutions to $f.$
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\begin{remark}
  If $g'$ is a general square subsystem of $f$, then it will have $d$ solutions and the only common solutions to $g$ and to
  $g'$ are solutions to $f$.
  In this case, if Algorithm~\ref{alg:set} returns FAIL, then $\#T>e$, so that some pair
  of balls in Step 6 meet, but their intersection does not contain a common solution to $g$ and to $g'$.
  In this case, we may then further refine the solutions in $S,S'$, and the corresponding balls until no such extraneous
  pair of balls meet.  
\end{remark}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\begin{remark}\label{Rem:Alg4_alternative}
  An alternate approach to this algorithm is to set up a linear parameter homotopy between
  $g$ and $g'$, which is natural if both are linear combinations of elements of $f$.
  Then the solutions which are in $\variety(f)$ are among those of $\variety(g)$ which do
  not move or leave the separating balls.
  If exactly $e$ solutions in $\variety(g)$ do not leave their separating nballs, then
  these are the solutions in $\variety(f)$.

  A proxy for this continuation is applying the Newton operator $N_{g'}$ to each
  point in $\variety(g)$.
\end{remark}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 



==> paper_bottom/circles.tex <==
Throughout, $v$ will denote the Gr\"{o}bner valuation defined by the graded lexicographical order with $y>x.$

Consider first the case $i=0.$ To compute $\Delta_{L_0},$ we may simply compute valuations of all polynomials in the $\CC$-span of $\{ f, g, h_0 \}.$ Note first that
\[
v(f) = v(h_0) = (0,0) \, \, \, \& \, \, \, v(g) = (1,0).
\]
To get more points in $v(L),$ we can take an ``S-pair'':
\[
S_1 := 7 f + 4 h_0 = 11 x^2 + 11 y^2 -24 x,
\]
which now has valuation $(1,0).$ Continuing,
\[
S_2 := 12 g - S_1 = x^2 + y^2 - 24 y,
\]
with valuation $(0,1).$ We have produced all valuations in $v(L)$---this is just a consequence of the fact that
\[
v(a) \ne v(b) \, \, \, \Rightarrow \, \, \, v(a+b) = \min \{ v(a), v(b) \} ,
\]
noting that $\{ S_2, f,g \}$ provide a basis of $L_0.$ Thus, the Newton-Okounkov body in this case is a lattice triangle in $\ZZ^2,$ with volume $1/2:$
\[
\Delta (A_{L_0}) = \conv \{ (0,0), (1,0), (0,1) \}
\]
Next, since the valuations $(1,0)$ and $(0,1)$ both appear at level 1, this implies $\ind A_{L_0} =1.$ Finally, we compute the degree of the Kodaira rational map:
\[
\Phi_{L_0}(x,y) = [x^2+y^2-4:x^2+y^2-2x-2y:x^2+y^2-6x+7].
\]
We have that
\[
\deg \Phi_{L_0} = \deg [k(x,y):\Phi^* 
\]
\red{Complete me}
We conclude
\[
[L_0:L_0] = 2! \cdot \frac{2}{1} \cdot (1/2) = 2.
\]
For the case of a single intersection, 
\red{Complete me}


==> paper_bottom/org.tex <==
\subsection{Organization of this paper}
\red{when finished}


==> paper_bottom/quarticSys.tex <==
\begin{align*}f_{1} &= z_1 \, z_2-z_2^2+z_1-z_2\\f_{2} &= z_1^2-z_2^2+4 \, z_1-4 \, z_2\\f_{3} &= z_2^3-6 \, z_2^2+5 \, z_2+12\\f_{4} &= z_1 \, z_2^2-6 \, z_2^2-z_1+6 \, z_2+12\\f_{5} &= z_1^2 \, z_2-6 \, z_2^2-4 \, z_1+9 \, z_2+12\\f_{6} &= z_1^3-6 \, z_2^2-13 \, z_1+18 \, z_2+12\\f_{7} &= z_2^4-31 \, z_2^2+42 \, z_2+72\\f_{8} &= z_1 \, z_2^3-31 \, z_2^2+z_1+41 \, z_2+72\\f_{9} &= z_1^2 \, z_2^2-31 \, z_2^2+4 \, z_1+38 \, z_2+72\\f_{10} &= z_1^3 \, z_2-31 \, z_2^2+13 \, z_1+29 \, z_2+72\\f_{11} &= z_1^4-31 \, z_2^2+40 \, z_1+2 \, z_2+72\end{align*}
